Software principles and concepts applied in the implementation of cyber-physical systems for real-time advanced process control

Cyber-physical systems (CPSs) for real-time advanced process control (RT-APC) are a class of control systems using network communication to control industrial processes. In this paper, we use simple examples to describe the software principles and concepts used in the implementation of such systems. The key software principles are 1) shared data in the form of a database, files, or shared memory, 2) timers and threads for concurrent periodic execution of tasks, and 3) network communication between the control system and the process, and communication between the control system and the internet, e.g., the cloud to enable remote monitoring and commands. We show how to implement such systems for Linux operating systems applying the C programming language and we also comment on the implementation using the Python programming language. Finally, we present a complete simulation experiment using a real-time simulator.

==> tex/old/code_and_listings.tex <==
\begin{algorithm}[tb]
\label{algo:generic_timer}
\caption{Generic timer with time drift correction}\label{alg:timer_sleep}

\KwData{Ts, callback()}
 \While{true}{
 t1 = getCurrentTime();\\
 callback();            \\
 t2 = getCurrentTime(); \\
 wait(Ts - (t2-t1));
 }
\end{algorithm}


\begin{algorithm}
\caption{Callback function: RT-simulation of plant}\label{alg:RT_sim}
\KwData{$x_k, u_k, d_k, p_f, p_g, f(\cdot), g(\cdot), n_x, T_s^p, N_s$}
\KwResult{$x_{k+1}, y_{k}$ and $t_{k}$ in UTC}
 Initialize $X\in\mathbb{R}^{N_s\times n_x}$\\
 // Get currenct timestamp (UTC)\\
 $t_k$ = gettimeofday(\&now)\\
 
 // Read most recent manipulated variables from server\\
 read($u_k$)
 
 // Compute measurements\\
 $y_k = g(t_k, x_k, u_k, d_k, p_g)$\\
 
 // Write measurements to server\\
 write($y_k$)\\
 
 // Simulate for $t_{k+1} = t_k+T_s^p$ \\
 $X, T = odesolver(f(t_k, x_k, u_k, d_k, p_f), [t_k, t_{k+1}], N)$\\
 $x_{k+1} = X(end)$


 
 
 
 
\end{algorithm}


\begin{figure}[tb]
\hspace{0.3cm}\begin{minipage}{0.46\textwidth}
\begin{lstlisting}[caption={Code for creating, starting, stopping, and deleting a timer for a control algorithm},label={lst:timer_code_control}, style=CStyle]
#include <stdio.h>
#include "apctimer.h"
// APC module
void cntrAlgo(union sigval sv){
    // Dereference pointer to timer data struct
    Args_apc* args = (Args_apc*)sv.sival_ptr;        
    /* Unpack dimensions ny, ny, nr, nI from args */
    
    /* Read y, r, and I from DB */

    /* Compute u using a control algorithm */
    
    /* get current time in UTC */
    
    /* Write u to DB */
    
    /* Update Controller */
}
int main(void){  
    // Create a timer for the control algorithm
    timer_t* td_apc = create_mytimer(cntrAlgo, args_apc);
    // Start the timer
    start_mytimer(td_apc, Ts_apc, 0.0,  NULL);
    // Sleep for 10 min
    sleep(600);
    // Stop the timer
    stop_mytimer(td_apc);
    // Delete the timer
    delete_mytimer(td_apc);
    return 0;
}
\end{lstlisting}
\end{minipage}\hfill\\
\end{figure}



% Timers
We design the function prototypes as  
\begin{minipage}{0.47\textwidth}
\begin{lstlisting}[style=CStyle]
timer_t create_mytimer(void (*fnc)(), void* args);
int start_mytimer(timer_t timerid, double Ts, double delay, char* abs_ts_str);
int stop_mytimer(timer_t timerid);
int delete_mytimer(timer_t timerid);
\end{lstlisting}
\end{minipage}\hfill\\








%% Shared Data listing

\begin{figure}[tb]
\centering
\begin{minipage}[tb!]{.47\textwidth}
\begin{lstlisting}[caption={Example code for initialization and modification of a table in a Shared Data using the PostgreSQL database system.},label={lst:db_code}, style=CStyle]
#include <stdio.h>
#include <libpq-fe.h>       
#include "apcshareddata.h" 

int main(int argc, char const* argv[]){
    char ts[27]; // timestamp
    // Create connection to PostgreSQL database (db)
    char conn_str[]  = "user=apc_user dbname=apc_db password=apc_password";
    PGconn *db_conn = PQconnectdb(conn_str);
    // Check connection to database
    checkStatus(db_conn);         
    // Init table in database for "sensor1"
    initTableFloat(db_conn, "sen", 1);
    genTimeStampUTC(ts);
    // Write to db (args: db conn, tablename, number, timestamp, status, value)
    insertIntoTableFloat(db_conn, "sen", 1, ts, "'ok'", 0.5);
    // Read data from last row of database
    double sen1_val = 0.0;
    char ts_str1[100], stat_str1[100]; 
    readRecentValFloat(db_conn, "sen",1, ts_str1, stat_str1, &sen1_val);
    // Close connection to db
    PQfinish(db_conn);
    return 0;
}
\end{lstlisting}
\end{minipage}\hfill\\
\end{figure}


==> tex/old/text.tex <==
%The POSIX timer API offer functionality for creating, starting, stopping, and deleting of POSIX interval timers. We use the CLOCK\_REALTIME as the clockid when creating a timer for configure the timer using system-wide real-time clock. The POSIX timer API offer the possibility to pass a notification function and additional arguments. This makes it possible to pass user defined callback functions with arguments for control algorithms, simulations, and other functions. Furthermore, by choosing the notification method as SIGEV\_THREAD this function can started in a new thread. This eliminates the tasks of manually creating threads for each periodic tasks.

%Another benefit of using these POSIX timers with thread invocation is the way the timer avoid time-drift. time-drift is the accumulation of excess time. A callback function do require takes time to execute and then the waiting time needs to be corrected. For thread invocation, the compuational time for one iteration do not affect the iteration of a second iteration. However, it is important that the computational time still do not exceed the interval time, as the number of threads then would accumulate.


requires a model in the form,
\begin{subequations}
\label{eq:RT_plant_sim_form}
\begin{alignat}{1}
        \dot x(t) &= f(t, x(t), u(t), p),\\
        y(t_k) &= g(t_k, x(t_k), u(t_k), p).
\end{alignat}
\end{subequations}


% In indtroduction
*** Introduction (ideas) *** 

- Advanced control of industrial processes enables, automatic, reliable, robust, and efficient operation.

- Advanced process control strategies such as model predictive control can further optimize the behavior of constrained systems. Especially, when forecasted disturbances or predefined changes in setpoints can be given directly to the algorithms.

- Cyber-physical systems (CPS) are systems that involves network communication, computers, and physical processes.

- The software aspects are crucial for development of automatic and efficient operation of CPS.

- The most important software principles and components used in the implementation of real-time advanced process control (RT-APC) for CPS are 1) shared data; 2) timers and multiple threads for periodic and concurrent execution of tasks; 3) network communication between the control system and the processes as well as the communication between the control system and the internet for remote monitoring and commands.

- Software frameworks that uses these principals and components also enables real-time simulation by using mathematical models of the processes. Consequently, these principals can applied to a proxy of the physical plant thus enabling real-time simulation of closed-loop system including the network communication.

- For client/server-based communication models, changing from real-time simulation to practical closed-loop control can be achieved by changing server endpoints.

- Previous work: real-time simulation, communication for control, timers and threads, databases and shared data for control. Generic and user friendly solutions [cite all these things]

- what is missing in research:

- (present novelty) In this paper we present software principles and concepts used in implementations of a generic RT-APC framework. We do this by presenting the different key components in such a framework for Linux operating systems using the C programming language and we showcase this framework through examples. These examples build gradually on top of each other and are based on custom libraries that serves as wrappers for the timer, database, and internet domain sockets APIs. In addition, we briefly outline the implementation using high-level programming languages. Finally, we tie all this examples together into a complete example for closed-loop control of a 1st-order linear model
simulated in real-time. The real-time simulation of the model and control system are communicating through a client/server-based model.




% In timers and threading
We use timers and threading principles for execution of concurrent and periodical tasks in a RT-APC framework. 
Typical tasks in a RT-APC framework may consist of 1) reading measurements from the Plant/Simulator to the Shared Data, 2) Reading measurements from the Shared Data to a Control Algorithm, 3) Compute and write control signals from the Control Algorithm to the Shared Data, 4) write control signals to the from the Shared Data to the Plant/Simulator. For efficient execution of tasks in a RT-APC framework the timers are required to functioning without accumulation of time drift. Additionally, the jitter, the difference between ideal and actual execution time, needs to be small compared to the computation time of the tasks to guarantee predictable behavior of the system.
Finally, interaction between an operator and the control system is also achieved using threading principals as setpoint or operation configurations should be delivered when when desired. However, these configurations might not need to be delivered using a timer-based approach.



% Communication

We use network communication principals for remote control and monitoring of Plants/Simulators. 
Transmission control protocol/internet protocol (TCP/IP) offer reliable exchange of data and we demonstrate how this protocol can be used in a Client/Server based communication model. We use internet domain stream sockets instead of OPC standard to demonstrate network communication in closed-loop control, as the basic principals for Client/Server based can be easily be shown through these examples. The internet domain stream sockets offer reliable and bidirectional based on the TCP/IP protocol
Automation pyramid\\

Industrial networks require
the transmission of both periodically sampled data and
aperiodic events such as change of state or alarm conditions [cite introduction to industrial control networks]. We limit the discussion to periodic transmission of state messages, e.g., control signals and sensor values that are updated periodically.

Data packets transmitted in industrial levels
are generally quite small - only a single measurement or digital value may
need to be transmitted, along with some overhead information.
Such transmissions are often only a few bytes in size, such as
the transmission of a single binary state or a sixteen bit value.

For industrial network, the main requirements are strong determinism and real-time data transfer.
\\
******\\

%In contrast to UPD/IP networking protocol, the TCP/IP is a connection-oriented communication method and requires a connection before messages can be exchanged.
%For internet domain stream sockets the connections between Clients and Servers are represented as file descriptors. We use these file descriptors to read and write N bytes of input into the memory area indicated by buf. 



\begin{table}[tb!]
\centering
\caption{Parameters for real-time simulation of linear 1st order system}
\label{tab:plant_simulator_parameters}
\begin{tabular}{lll}
\hline
Parameters & Value & Unit \\ \hline
$K$         &    10.0  & - \\
$\tau$        &    10.0 &-  \\
$T_s^{p}$         &  0.5  & s  \\ \hline
\end{tabular}
\end{table}

\begin{table}[tb!]
\centering
\caption{Parameters for PI-controller}
\label{tab:PI_parameters}
\begin{tabular}{lll}
\hline
Parameters & Value & Unit \\ \hline
$K_p$         &    0.2  & - \\
$\tau_i$        &    10.0 & -  \\
$T_s^{c}$         &  2.0   & s  \\ 
$\bar{u}_k$      & 0.0       & -\\ \hline
\end{tabular}
\end{table}
\begin{figure}[tb]
    \centering
    \includegraphics[width=0.485\textwidth]{fig/timing.pdf}
    \caption{The timing diagram of the real-time execution of the tasks for the Control module in Fig. \ref{fig:timers_and_threads} with sampling jitter.}
    \label{fig:timing}
\end{figure}

Fig. \ref{fig:timing} illustrates the the sampling jitter e.g., the variation in sampling interval and the
computational delay jitter of the Control Module in Fig. \ref{fig:timers_and_threads} \cite{Wittenmark:Aastrom:Arzen:2022}.


\subsection{Discussion the results}

- natural delay in control due to the communication layer. The measurement data from the plant needs to be sampled and send to the database. 






